A Receding-Horizon MDP Approach for Performance Evaluation of Moving Target Defense in Networks

In this paper, we study the problem of assessing the effectiveness of a proactive defense-by-detection policy with a network-based moving target defense. We model the network system using a probabilistic attack graph--a graphical security model. Given a network system with a proactive defense strategy, an intelligent attacker needs to perform reconnaissance repeatedly to learn about the locations of intrusion detection systems and re-plan optimally to reach the target while avoiding detection. To compute the attacker's strategy for security evaluation, we develop a receding-horizon planning algorithm using a risk-sensitive Markov decision process with a time-varying reward function. Finally, we implement both defense and attack strategies in a synthetic network and analyze how the frequency of network randomization and the number of detection systems can influence the success rate of the attacker. This study provides insights for designing proactive defense strategies against online and multi-stage attacks by a resourceful attacker.

==> archieve.tex <==

\section{Preliminaries}


Notation: Given a finite set $X$, let $\Delta(X)$ be the set of probability distributions over $X$. The size of the set $X$ is denoted by $\abs{s}$. Let $\Sigma$ be an alphabet (a finite set of symbols). Given $k \in \nat^{+}$, $\Sigma^k$ indicates a set of words with length $k$, $\Sigma^{\leq k}$ indicates a set of words with length smaller than or equal to $k$, and $\Sigma^0 = \lambda$ is the empty word. $\Sigma^\ast$ is the set of finite words (also known as Kleene closure of $\Sigma$), and $\Sigma^\omega$ is the set of infinite words.  $\indicator_X$ is the indicator function with $\indicator_X(x) =1, \text{ if } s \in X$ and $0$ otherwise.


\subsection{Syntactically co-safe Linear Temporal Logic}
Syntactically co-safe \ac{ltl} formulas~\cite{Kupferman2001} are a well-defined subclass of \ac{ltl} formulas. Given a set of atomic propositions $\calAP$, the syntax of \ac{scltl} formulas is defined as follows:
\begin{equation*}
    \varphi \coloneqq \BoolTrue \mid p \mid \neg p \mid \varphi_1 \wedge \varphi_2 \mid \Next \varphi \mid \varphi_1 \Until \varphi_2,
\end{equation*}
where $\varphi, \varphi_1$ and $\varphi_2$ are \ac{scltl} formulas, $\BoolTrue$ is the unconditional true, and $p$ is an atomic proposition. Negation ($\neg$), conjunction ($\wedge$), and disconjunction ($\vee$) are standard Boolean operators. A \ac{scltl} formula can contain temporal operators \say{Next} ($\Next$), \say{Until} ($\Until$), and \say{Eventually} ($\Eventually$). However, temporal operator \say{Always} ($\Always$) is not contained in \ac{scltl}.

An infinite word with alphabet $2^\calAP$ satisfying a \ac{scltl} formula always has a finite-length good \emph{prefix}~\cite{Kupferman2001}~\footnote{$u$ is a prefix of $w$, \ie, $w=uv$ for $u, v\in\Sigma^\ast$}. Formally, given a \ac{scltl} formula $\varphi$ and an infinite word $w = r_0 r_1 \cdots $ over alphabet $2^{\calAP}$, $w \models \varphi$ if there exists $n \in \naturals$, $w_{[0:n]} \models \varphi$, where $w_{[0:n]} = r_0 r_1 \cdots r_n$ is the length $n+1$ prefix of $w$. Thus, an \ac{scltl} formula $\varphi$ over $2^\calAP $ can be translated into a \ac{dfa} $\calA_{\varphi} = \langle Q, \Sigma, \delta, q_0, F \rangle$, where $Q$ is a finite set of states,  $\Sigma = 2^{\calAP}$ is a finite set of symbols called the alphabet, $\delta: Q \times \Sigma \rightarrow Q$ is a transition function, $q_0\in Q$ is  an initial  state, and $F\subseteq Q$ is a set of accepting states. A transition function is recursively extended in the general way: $\delta(q,aw)=\delta( \delta(q,a),w )$ for given $a\in \Sigma$ and $w\in \Sigma^\ast$. A word $w = uv$ is \emph{accepting} if and only if $\delta(q, u)\in F$. \ac{dfa} $\calA_\varphi$ accepts the set of words satisfying $\varphi$.

We consider stochastic systems modeled as \ac{mdps}. We introduce a labeling function to relate paths in an \ac{mdp} $M$ to a given specification described by an \ac{scltl} formula.

\begin{definition}[Labeled \ac{mdp}]
\label{def:labeled_mdp}
	A labeled \ac{mdp} is a tuple $M = \langle S, A, s_0, P, \calAP, L \rangle$, where $S$ and $A$ are finite state and action sets, $s_0$ is the initial state, the transition probability function $P(\cdot \mid s, a) \in \Delta(S)$ is defined as a probability distribution over the next state given action is taken at the current state, $\calAP$ denotes a finite set of atomic propositions, and $L: S \rightarrow 2^{\calAP}$ is a labeling function mapping each state to the set of atomic propositions true in that state.
\end{definition}

A finite-memory stochastic policy in the \ac{mdp} is a function $\pi: S^{\ast} \rightarrow \Delta(A)$ that maps a history of state sequence into a distribution over  actions. A Markovian stochastic policy in the \ac{mdp} is a function $\pi: S \rightarrow \Delta(A)$ that maps the current state into a distribution over actions. Given an \ac{mdp} $M$ and a policy $\pi$, the policy induces a Markov chain $M^{\pi} = \{s_t \mid t = 0, \dots, \infty \}$ where $s_i$ is the random variable for the $i$-th state in the Markov chain $M^{\pi}$, and it holds that $s_{i+1} \sim P(\cdot \mid s_i, a_i)$ and $a_i \sim \pi(\cdot \mid s_0 s_1 \ldots s_i)$.

Given a finite (resp. infinite) path $\rho  =s_0s_1\ldots s_N \in S^\ast$ (resp. $\rho \in S^\omega$), we obtain a sequence of labels $L(\rho) = L(s_0)L(s_1)\ldots L(s_N)\in \Sigma^\ast$ (resp. $L(\rho) \in \Sigma^\omega$). A path $\rho$ satisfies the formula $\varphi$, denoted by $\rho \models \varphi$, if and only if $L(\rho) $ is accepted by $\calA_\varphi$. Given a Markov chain induced by policy $\pi$, the probability of satisfying the specification, denoted by $P(M^\pi\models \varphi)$, is the expected sum of the probabilities of paths satisfying the specification.
\[
P(M^\pi \models \varphi) \coloneqq \Expect\left[\sum_{t=0}^\infty \indicator(\rho_t\models \varphi)\right],
\]
where ${\rho}_t =s_0s_1\ldots s_t$ is a path of length $t+1$ in $M^\pi$. 

\subsection{Finite-horizon risk-averse planning}
\jf{here: please include necessary prelim. Can reuse the structure of MDP above.}

\subsection{Problem formulation}
\jf{stating the problem}
\begin{problem}
Given an \ac{mdp} $M$ and a time varying labeling function $L_t$ with unknown dynamics, develop an algorithm for online planning.
\end{problem}
\jf{this problem statement is incomplete. what is the notion of optimality? how to measure the performance of your algorithm?}

\normalcolor
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Linear temporal logic (LTL) specifications are sufficient to express a wide range of system properties such as satey, reachability, obligation, stability, and liveness \cite{manna2012temporal}. The two main limitations towards practical applications of LTL specifications are: 1) The state explosion problem \cite{piterman2006synthesis}: It is often necessary to generate a finite state automata from LTL specifications to keep track of the evolution of state variables with respect to LTL specifications. The states in the automata, also referred to as the memory states, grow exponentially in the length of a specification \cite{gastin2001fast} and thus limits the application of LTL synthesis to relatively small problems. 2) The lack of flexibility: With a small change in the specification or environment, a new policy may need to be synthesized from scratch.

To alleviate the associated scalability of LTL synthesis, we exploit the idea of composition planning in Markov decision process (MDP) \cite{silver2012compositional, bacon2017option, liu2019compositional}. To accomplish complex tasks, composition allows planning with macro-actions—policies for simple subtasks—with different time scales. The tasks expressed in LTL specifications are first decomposed into a small set of subtasks. Once the macro-actions for the sub-tasks are computed by the agent, they are augmented with the original action set to compose the global optimal or near optimal policy. 

To improve flexibility for planning complex tasks, we apply an idea similar to the traditional receding horizon control \cite{wongpiromsarn2012receding}. In the controls domain, receding horizon control is an effective and well-established technique to address this issue. This control approach optimizes over a shorter horizon, starting from the currently observed state, implements the initial control action, moves the horizon one step ahead, and re-optimizes. A technology similar to receding horizon control, namely finite horizon risk sensitive MDP, is used in our project to compute the macro-actions for subtasks. Since it essentially solves a smaller optimization problem with a specific initial condition, change in initial condition (such as environment, goal, initial location) wouldn't affect execution of the controller. Therefore, receding horizon control improves flexibility for planning. In contrast, infinite horizon planning requires a new policy to be generated after the initial condition changes or optimizing with all possible initial conditions to begin with. 

In conclusion, this project aims to reduces a complex tasks into a set of smaller problems of short horizon while preserving the desired system-level temporal properties after composition.
\todo[inline]{literature survey first:}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}

\end{example}
\paragraph*{The attacker's objective: } Let $\calAP$ be a set of atomic propositions and a labeling function $L: V\rightarrow 2^\calAP$ maps a state in the network to a set of atomic propositions evaluated true at that state.

We assume that the attacker's objective is given by a co-safe \ac{ltl} formula $\varphi$ that captures the objective of lateral movement attack and stealthy attack. The goal with  lateral movement attack, expressed by a co-safe \ac{ltl} formula $\varphi_L$, describes a temporal sequence of hosts to be visited.  The goal with stealthy attack, expressed by an invariant property $\varphi_S$, describes a set of hosts to be avoided in order to remain undetected by the defender. For example, $\varphi_S \coloneqq \neg \mbox{ids}$ means that the attacker intends to avoid all intrusion detection systems in  the network.

The task specification of the attacker is $\varphi_S\Until \varphi_L$--that is, the attacker is to remain stealthy until achieving the attack objective.

The following assumption  is made about the information and knowledge of the attacker.
\begin{itemize}
\item The attacker knows the set $V$ of states in the network but does
  not know the set of different configurations, represented by the set
  $\{E_i\mid i \in I\}$.
%\item The attacker knows \emph{partially} the labeling function $L$. For example, the attacker knows which states to reach in order to achieve the desired attack objective, but may not know partially the location of the IDS system. 
\item The attacker knows the labeling function $L$. 
\end{itemize}


  The goal is to verify the security of the network system given the \ac{mtd} policy. Given the attacker's incomplete knowledge about the network system, we assume that the attacker carries out online planning methods in the stochastic system.
  \begin{problem}
    Given the network system with a set $I$ of different configurations and an  \ac{mtd} policy that switches between different configurations, assume that  an attacker that plans online to satisfy the \ac{ltl} specification $\varphi$, verify if the system is secure with probability $\ge \epsilon$, for a pre-defined constant $\epsilon \in (0,1]$.  
  \end{problem}


  \begin{example}
  \zhu{What does this small network look like? It is a network with 5 nodes? More details would be useful.}
Consider a small network with two configurations in Fig.~\ref{fig:networksys_ex}. The attacker actions $a_1,a_2,a_3,a_4$ have different probability of success $p_1,p_2,p_3,p_4$. When an action fails, the attacker remains in the same state. In this network, if the attacker reaches states  $H_1$ and $H_5$, then he will be detected by the intrusion detection systems.  The \ac{mtd} policy is described as follows: For every $k$ time steps, the system will switch its configuration according to the following distribution $d: I \rightarrow[0,1]$ with $d(1)= \alpha$, and $d(2)=1-\alpha$. Here,  $\{p_i,i=1,\ldots, 4\}, k, \alpha$ are parameters of the network. 
\begin{figure}[htb]
  \begin{subfigure}[b]{0.5\textwidth}
    \input{./figs/networkconf1.tex}
    \caption{The  attack graph with probabilistic transitions given the network configuration 1.}

    \end{subfigure}
    \begin{subfigure}[b]{0.5\textwidth}
      \input{./figs/networkconf2.tex}
          \caption{The  attack graph with probabilistic transitions given the network configuration 2.}
        \end{subfigure}
        \caption{A network system with two different configurations.}
        \label{fig:networksys_ex}
      \end{figure}

      The attackder's objective is $\varphi_S\Until \varphi_L$ where
      $\varphi_L = \Eventually (S_1\land \Eventually S_2)$ and
      $\varphi_S = \neg \mbox{ids}$. The labeling function
      $L (S_i)=S_i$, $L(H_2)=L(H_5)= \mbox{ids}$.
    \end{example}
\todo[inline]{end of the new example.}
    \newpage



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
[RHC]

The attacker's receding horizon policy is computed by solving the risk-sensitive MDP. The MDP is built upon the network graph, its states set $S$ corresponds to all the nodes in the network, its action set $A$ corresponds to every types of system vulnerability. \jf{The receding horizon algorithm is presented in Alg. \ref{alg: RHC}, with explanations of the parameters and key steps as follows.}

The transition probability is feed as input to Alg. \ref{alg: RHC}, which is the probability of the attacker successfully exploits a vulnerability. The output of Alg. \ref{alg: RHC} is the policy $\pi_t$ for the attacker at time instant $t$. At the beginning of the while loop (line 2 in Alg. \ref{alg: RHC}), the algorithm would check if the attacker has been detected, has the attacker reached the target or has the time instant $t$ exceed maximum $t_{\max}$. The last constraint is put to avoid a endless loop.  

Since a roaming decoys policy is used by the network system, the attacker does not have full knowledge of the decoys trajectory. In light of that, the attacker would assume  the  decoy  is  static  through  the entire  time  horizon  of  an  online  iteration set the instant cost to be a function of state and action only. Value $V(x_{dec})$ is assigned to the decoys states and Value $V(x_{tar})$ is assigned to the target states. The instant cost $r_t(s,a)$ is updated using the following formula (line 4 in Alg. \ref{alg: RHC}): 
\begin{equation}
\begin{split}
r_t(s,a) & = r(s,a)\\
& = p(tar|s,a)V(x_{tar}) + p(dec|s,a)V(x_{dec})
\end{split}
\end{equation}

Given the reward $r_t(s,a)$, we can compute the receding horizon policy by solving the dual linear program defined in Eq. (10) (line 5 in Alg. \ref{alg: RHC}). After the computed attack action is carried out, the horizon is moved one step ahead (line 3 in Alg. \ref{alg: RHC}).

==> figs/networkconf1.tex <==



\begin{tikzpicture}[shorten >=1pt,node distance=3cm,on grid,auto, scale=0.6,every node/.style={transform shape}] 
   \node[state, initial] (0)   {$H_0$}; 
   \node[state, fill=red!20] (1) [  right = of 0] {$H_1$};
   \node[state] (2) [ below   =of 1] {$H_2$};
   \node[state] (3)  [  right =of 1]  {$S_1$};
   \node[state] (4)  [ right=of 3]  {$H_4$};
 
   \node[state, fill=red!20] (5)  [ below =of 4]  {$H_5$};
   \node[state] (6)  [ right =of 4]  {$H_6$};
   \node[state] (7)  [ right =of 5]  {$S_2$};

   \path[->] 
    (0) edge node{$a_1:p_1$} (1)
    (0) edge node[right]{$a_2:p_2$} (2)
    (1) edge node{$a_2:p_2$} (2)
    (2) edge node[right]{$a_1:p_1$} (3)
    (3) edge node{$a_1:p_1$, $a_2:p_2$} (4)
    (4) edge node{$a_1: p_1$} (6)
    (5) edge node[right]{$a_2:p_2$} (6)
    (4) edge node{$a_2:p_2$} (5)
    (6) edge node{$a_1:p_1$} (7);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> figs/networkconf2.tex <==



\begin{tikzpicture}[shorten >=1pt,node distance=3cm,on grid,auto, scale=0.6,every node/.style={transform shape}] 
   \node[state, initial] (0)   {$H_0$}; 
   \node[state, fill=red!20] (1) [  right = of 0] {$H_1$};
   \node[state] (2) [ below   =of 1] {$H_2$};
   \node[state] (3)  [  right =of 1]  {$S_1$};
   \node[state] (4)  [ right=of 3]  {$H_4$};
 
   \node[state, fill=red!20] (5)  [ below =of 4]  {$H_5$};
   \node[state] (6)  [ right =of 4]  {$H_6$};
   \node[state] (7)  [ right =of 5]  {$S_2$};

   \path[->] 
    (0) edge node{$a_3:p_3$} (1)
    (1) edge node{$a_4:p_4$} (2)
    (2) edge node[right]{$a_3:p_3$} (3)
    (3) edge node{ $a_4:p_4$} (5)
    (3) edge node{ $a_3:p_3$} (4)
    (4) edge node{ $a_4:p_4$} (5)
    (5) edge node[right]{$a_3:p_3$} (6)
    (5) edge node{$a_4:p_4$} (7)
    (6) edge node {$a_3:p_3$} (7);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> intro.tex <==

 
